Simulation of the Lattice QCD and Technological Trends in Computation

Simulation of Lattice QCD is a challenging computational problem. Currently, technological trends in computation show multiple divergent models of computation. We are witnessing homogeneous multi-core architectures, the use of accelerator on-chip or off-chip, in addition to the traditional architectural models. On the verge of this technological abundance, assessing the performance trade-offs of computing nodes based on these technologies is of crucial importance to many scientific computing applications. In this study, we focus on assessing the efficiency and the performance expected for the Lattice QCD problem on representative architectures and we project the expected improvement on these architectures and their impact on performance for Lattice QCD. We additionally try to pinpoint the limiting factors for performance on these architectures.

==> Makefile <==
TARGET=QCDTech
# Sources
SRCS=abstract.tex acknowledgements.tex cell.tex comparison.tex conclusion.tex gpu.tex singlenode.tex introduction.tex itanium.tex LQCD.tex pentium.tex multinode.tex
PAPER_SIZE = a4
IMGS=CellBE-comm.pdf Para-paper-02-figb2.pdf Fusedcomputation.pdf Cell_perf.pdf CPU-GPU.pdf GPUgranularity.pdf GPUgflops.pdf Interconnect.pdf gflopsvalid.pdf ia64_perf.pdf HoppingMatrix.pdf Para-paper-02-figa2.pdf Summary-attrib.pdf

EXTENSION=aux toc idx ind ilg log out lof lot lol bbl blg

all: ${TARGET}.pdf


%.pdf: %.tex
	pdflatex $<
	bibtex `basename $< .tex`
	pdflatex $<
	pdflatex $<

QCDTech.pdf: ${SRCS} ${IMGS}

# DeViceIndependent
#${TARGET}.pdf: ${SRCS}
#	echo "Running latex..."
#	latex ${TARGET}.tex
#	echo "Running bibtex..."
#	bibtex ${TARGET}
#	echo "Rerunning latex...."
#	latex ${TARGET}.tex
#	latex_count=5 ; \
#	while egrep -s 'Rerun (LaTeX|to get cross-references right)' ${TARGET}.log && [ $$latex_count -gt 0 ] ;\
#	    do \
#	      echo "Rerunning latex...." ;\
#	      latex ${TARGET}.tex ;\
#	      latex_count=`expr $$latex_count - 1` ;\
#	    done
#	dvips -o ${TARGET}.ps ${TARGET}.dvi 
#	ps2pdf ${TARGET}.ps ${TARGET}.pdf 

# Clean
clean:
	for EXT in ${EXTENSION}; \
	do \
	find `pwd` -name \*\.$${EXT} -exec rm -v \{\} \; ;\
	done
	rm -f ${TARGET}.dvi
	rm -f ${TARGET}.pdf
	rm -f ${TARGET}.ps	


==> powerpc.tex <==
\subsection{\label{sec:PowerPCSystems}PowerPC-based systems}

PowerPC processor is used in building the BlueGene family of supercomputing facilities.
BlueGene is scalable massively parallel systems
targeting challenging scientific computations. The latest generation,
BlueGene/P, is based on Power6 architecture. The Power6 architecture
embeds quad PowerPC 450 cores, at 850 Ghz, in a single chip with L3
cache of 8 MB. The bandwidth to the memory is 13.6 GBytes/s, adopting
the memory controller on chip methodology. The Power6 architecture
implements complex arithmetic instructions that are important for
the computations of the Lattice QCD. Blue gene implements 3D Torus
communication architecture with 12 unidirectional 450~MB/s links. 

BlueGene is considered today as the best architecture for LQCD
and many groups use it and study steadily the possible
improvements~\cite{Vranas06,Doi07}. The efficiency of the Lattice QCD 
computation on these systems is in the range of 20\%~\cite{Vranas06}.
We will not cover further this issue in this paper.
